A Framework for Vehicle Routing Approximation Schemes in Trees

We develop a general framework for designing polynomial-time approximation schemes (PTASs) for various vehicle routing problems in trees. In these problems, the goal is to optimally route a fleet of vehicles, originating at a depot, to serve a set of clients, subject to various constraints. For example, in Minimum Makespan Vehicle Routing, the number of vehicles is fixed, and the objective is to minimize the longest distance traveled by a single vehicle. Our main insight is that we can often greatly restrict the set of potential solutions without adding too much to the optimal solution cost. This simplification relies on partitioning the tree into clusters such that there exists a near-optimal solution in which every vehicle that visits a given cluster takes on one of a few forms. In particular, only a small number of vehicles serve clients in any given cluster. By using these coarser building blocks, a dynamic programming algorithm can find a near-optimal solution in polynomial time. We show that the framework is flexible enough to give PTASs for many problems, including Minimum Makespan Vehicle Routing, Distance-Constrained Vehicle Routing, Capacitated Vehicle Routing, and School Bus Routing, and can be extended to the multiple depot setting.

==> tex/chen_marx.tex <==

\section{Chen and Marx's Previous Claim to a Minimum Makespan PTAS}\label{sec:chen_marx}

A recent paper of Chen and Marx~\cite{chen_marx} claims to present a PTAS for {\sc Minimum Makespan Rooted Tree Cover}.  In this section we show that their theorem (Theorem 2.1~\cite{chen_marx}) is incorrect.  Additionally, we compare their approach to our own and describe how we successfully overcome the challenges where their approach fell short.

The intuition behind our result is similar to that of~ \cite{chen_marx}: since the main challenge arises from having to account for small tour segments, modify the instance so that only large tour segments need to be accounted for.  Because each tour can only have a small number of these larger tour segments, the algorithm can essentially \emph{guess} all possible ways that the segments can be joined to form tours.  The difficulty with this approach is in showing that this type of grouping of small segments into large segments can be done without incurring too much error.
%
As did~\cite{chen_marx}, we also observed that assuming each subtree with length less than $\ep OPT$ to be covered by a single tour increases the makespan by $O(\ep OPT)$, where $OPT$ is the optimum makespan.  


Their Theorem 2.1~\cite{chen_marx} (which their PTAS requires) depends on the following argument, though they use different terminology: Let $T_v$ denote the subtree rooted at $v$.  The input can be \emph{safely} modified\footnote{\emph{Safe} graph modifications are those that result in an equivalent instance and consist  of subdividing a single edge $e_0$ into two smaller edges $e_1$ and $e_2$ such that $\ell(e_1) + \ell(e_2) = \ell(e_0)$.} so that there exists a set of vertices $CR$ such that the subtrees rooted at vertices in $CR$ collectively \emph{partition} the leaves of the tree and such that $CR$ has the following properties:

\begin{enumerate} %[label =  (\roman*)]
%\setlength{\itemsep}{0pt}
\item For each $v\in CR$, $T_v$ is \emph{small}: for each child $u$ of $v$, the length of $T_u$ is less than $\ep OPT$.
\item For each $v\in CR$, $T_v$ is \emph{large}: the length of $T_v$ is at least $\ep OPT$.
\item The vertices of $CR$ are \emph{independent}: no two distinct vertices in $CR$ have an ancestor-descendant relationship.
\end{enumerate}

Each of these properties is vital to the proof of Theorem 2.1~\cite{chen_marx}: Property 1 bounds the solution error, Property 2 ensures polynomial runtime, and Property 3 ensures solution feasibility.

Given such a set $CR$, Chen and Marx~\cite{chen_marx} prove that there exists a near-optimal solution in which each \emph{branch} of a subtree rooted at a vertex in $CR$ is covered by a single tour.  They do so by showing that an optimal solution $SOL$ can be transformed into a near-optimal solution $SOL'$ in which each such branch is wholly covered by one of the tours that partially covers it in $SOL$.  This proof depends on Property 1 to bound the resulting error of this transformation and on Property 3 to maintain solution feasibility while independently reassigning branch coverage.  A dynamic programming strategy can then be used to find such a near-optimal solution, which requires Property 2 in order to achieve a polynomial runtime.

The problem, though, is that no such set $CR$ is guaranteed to exist. In the process of modifying the input graph to ensure that their proposed set $CR$ satisfies Property 3, they end up with a set that no longer satisfies Property 2.  

In fact, it is not difficult to show the following.

\begin{lemma}
\label{lem:chen_marx}
There exist instances in which no such set $CR$ as described above exists.
\end{lemma}
\begin{proof}
We describe an instance that neither admits such a set $CR$ nor can be modified using \emph{safe} graph modifications into an equivalent instance that admits such a set. Let $T$ be a tree with root $r$ that consists of a \emph{central} path $P = r, v_1, v_2, ..., v_{l}$, \emph{side} subtrees $T_i$ for $i \in \{1,2,...,l\}$ such that the root of $T_i$ is a child of $v_i$, and \emph{main} subtree $T_{l+1}$ whose root $v_{l+1}$ is a child of $v_l$. Let edges $(v_i,v_{i+1})$ along $P$ have small nonzero lengths, let each side subtree $T_i$ have total length less than $\frac{\ep OPT}{2}$ and let the main subtree $T_{l+1}$ have total length at least $\frac{\ep OPT}{2}$ (see Figure~\ref{fig:counter}).  In order to satisfy Property 2, no vertex $v$ in any side subtree $T_i$ for $0<i\leq l$ can be in $CR$, since the subtree rooted at such a $v$ is not large enough.  So, since the subtrees rooted at vertices in $CR$ partition the leaves of $T$, at \emph{least} one vertex in $P$ must be in $CR$ to cover the leaves of trees $T_i$.  At the same time, in order to satisfy Property 3, at \emph{most} one vertex in $P$ can be in $CR$.  But, since main subtree $T_{l+1}$ is large, no choice of vertex in $P$ can satisfy Property 1.

Note that the side and main subtrees are general, and can be assumed to be defined after any safe modifications occur.  Additionally, if any edges of $P$ are subdivided, the argument above clearly still holds.

\begin{figure}[!h]
\centering
      \includegraphics[width=.5\textwidth]{figures/counter2}
\caption{\label{fig:counter} Counterexample to~\cite{chen_marx}.}
\end{figure}
\end{proof}

The counterexample in the above proof allows an arbitrarily complex and heavy main subtree $T_{l+1}$, so it cannot be argued that only trivial examples fail to admit a set $CR$.  In particular, this pattern of light side subtrees can continue throughout the main subtree, so these \emph{difficult areas} cannot be easily dealt with separately.


To the best of our knowledge, there is no straightforward way to salvage the theorem used in \cite{chen_marx}.  In fact, the crux of the problem is highlighted by the \emph{absence} of such a set $CR$: How can the input be simplified so as to balance error with runtime given that coverage choices are \emph{not} independent?  Our approach uses similar intuition to that of~\cite{chen_marx}, but manages to successfully address the critical challenges of the problem where prior attempts have fallen short.


Rather than partition the tree uniformly into subtrees, we recognize that the behavior of solutions \emph{looks} differently near the leaves than it does along internal vertices.  As such, our framework partitions the \emph{entire} tree into three different types of \emph{clusters} (see Figure~\ref{fig:clusters}).  \emph{Leaf clusters} are defined greedily so as to satisfy properties similar to 1-3 above and serve to anchor the cluster structure.  \emph{Small clusters} are internal clusters with weight (and frequency) small enough to be effectively ignored while incurring only a small error that can be \emph{charged} to the leaf clusters.  The remainder of the tree is grouped into \emph{edge clusters}, with properties similar to 1 and 2 above: their weight is \emph{small} enough to assume, without incurring too much error, a \emph{simple} structure to the way that tours cover them, yet they are \emph{large} enough so that any tour can only cover a bounded number of them. Though the edge clusters themselves do \emph{not} maintain independence, we show a weaker, sufficient property exhibited by tour segments in these clusters that ensures tour connectivity while treating edge clusters independently.
